Anatomy of a High-Profile Data Breach: Dissecting the Aftermath of a Crypto-Wallet Case

Media reports show an alarming increase of data breaches at providers of cybersecurity products and services. Since the exposed records may reveal security-relevant data, such incidents cause undue burden and create the risk of re-victimization to individuals whose personal data gets exposed. In pursuit of examining a broad spectrum of the downstream effects on victims, we surveyed 104 persons who purchased specialized devices for the secure storage of crypto-assets and later fell victim to a breach of customer data. Our case study reveals common nuisances (i.e., spam, scams, phishing e-mails) as well as previously unseen attack vectors (e.g., involving tampered devices), which are possibly tied to the breach. A few victims report losses of digital assets as a form of the harm. We find that our participants exhibit heightened safety concerns, appear skeptical about litigation efforts, and demonstrate the ability to differentiate between the quality of the security product and the circumstances of the breach. We derive implications for the cybersecurity industry at large, and point out methodological challenges in data breach research.

==> fig/data/harm <==
%file=../Latex/descriptive/data/harm, n_bars=15, max_value=93
%names:, Scam, Marketing, Password request, Ransom/threat, Scam letter, Account control attempt, Account control success, New account attempt, New account success, No harm, Cyberbullying, SIM swap attempt, SIM swap success, Fake hardware wallet received, Physical threats, 
\draw (1,0)--(1,93*100/104) node[above=-4pt, black] {93}
(2.2,0)--(2.2,82*100/104) node[above=-4pt, black] {82}
(3.4,0)--(3.4,54*100/104) node[above=-4pt, black] {54}
(4.6,0)--(4.6,33*100/104) node[above=-4pt, black] {33}
(5.8,0)--(5.8,22*100/104) node[above=-4pt, black] {22}
(7,0)--(7,19*100/104) node[above=-4pt, black] {19}
(8.2,0)--(8.2,2*100/104) node[above=-4pt, black] {2}
(9.4,0)--(9.4,17*100/104) node[above=-4pt, black] {17}
(10.6,0)--(10.6,6*100/104) node[above=-4pt, black] {6}
(11.8,0)--(11.8,5*100/104) node[above=-4pt, black] {5}
(13,0)--(13,4*100/104) node[above=-4pt, black] {4}
(14.2,0)--(14.2,3*100/104) node[above=-4pt, black] {3}
%(15.4,0)--(15.4,0*100/104) 
(15.4,0)--(15.4,2*100/104) node[above=-4pt, black] {2}
(16.6,0)--(16.6,2*100/104) node[above=-4pt, black] {2}; 

==> fig/data/protec <==
%file=../Latex/descriptive/data/protec, n_bars=18, max_value=54
%names:, I started using (or significantly extended the use of) multi-factor authentication for my online accounts., I changed/updated a password for my e-mail account., I started using (or significantly extended the use of) authenticator apps., I changed/updated a password for my account(s) related to crypto assets., I notified others who may also have been affected by the breach., I started (or significantly extended the use of) using a password manager., I relocated my recovery seed phrase to another, more secure physical place., I transferred my crypto assets stored on the hardware wallet to another crypto wallet., I relocated my hardware wallet to another, more secure physical place., I improved my home security (e.g., by installing a visual security alarm system, updating locks, investing in a safe etc.)., I did not take any actions., I started using (or significantly extended the use of) the hardware-based multi-factor authentication (e.g, Yubikey, Titan), I transferred my crypto assets stored on an exchange to another crypto wallet., I contacted my telecom provider to prevent SIM swapping attacks., I asked other companies to delete my personal data or online accounts., Idk, Increased awareness, Other, 
\draw (1,0)--(1,54) node[above=-4pt, black] {54}
(2,0)--(2,49) node[above=-4pt, black] {49}
(3,0)--(3,46) node[above=-4pt, black] {46}
(4,0)--(4,43) node[above=-4pt, black] {43}
(5,0)--(5,34) (6,0)--(6,34) (7,0)--(7,28) (8,0)--(8,22) (9,0)--(9,19) (10,0)--(10,18) (11,0)--(11,17) (12,0)--(12,12) (13,0)--(13,12) (14,0)--(14,12) (15,0)--(15,11) (16,0)--(16,4) (17,0)--(17,4) (18,0)--(18,0) ;

==> fig/data/response <==
%file=../Latex/descriptive/data/response, n_bars=16, max_value=47
%names:, Company advice, Followed disc. online, Time, Followed disc. website, Sought advice online, Sought advice community, No need, Shared exp. online, Sought advice peers, Sought advice company, Sought advice expert, I could not do anything., Spam management, Police, Other, I don't know, 
\draw (1,0)--(1,47) node[above=-4pt, black] {47}
(2,0)--(2,40) node[above=-4pt, black] {40}
(3,0)--(3,37) node[above=-4pt, black] {37}
(4,0)--(4,33) node[above=-4pt, black] {33}
(5,0)--(5,20) (6,0)--(6,17) (7,0)--(7,16) (8,0)--(8,13) (9,0)--(9,11) (10,0)--(10,9) (11,0)--(11,4) (12,0)--(12,3) (13,0)--(13,3) (14,0)--(14,2) (15,0)--(15,2) (16,0)--(16,2) ;

==> fig/harm.tex <==

	%min and max values
\def\xmax{14.6}
\def\ymax{100}
\def\xmin{0.25}

 
\begin{tikzpicture}[xscale=0.75, yscale=0.037, answer/.style={anchor=north east, align=right,rotate=45, text width=3cm}]

	%data
	\begin{scope}[line width=12, maincolor]
		\input{./data/harm}
	\end{scope}

	%axis
	\draw[<->] (\xmin, \ymax) -- (\xmin, 0) -- (\xmax, 0);
	
	%x-axis
	\foreach[count=\i] \harm in {Scam, Marketing, Password request, Ransom/threat, Scam letter, Account control attempt}
		{
			\draw (\i,0) node[below,answer] {\scriptsize \harm};}
	
	\draw (6.6,0) node[below,answer] {\scriptsize Account control success};
	\draw (7.6,0) node[below,answer] {\scriptsize New account attempt};
	\draw (8.2,0) node[below,answer] {\scriptsize New account success};
	
	\foreach[count=\i] \harm in {No harm, Cyberbullying, SIM swap attempt}
	{
		\draw (8.2+\i,0) node[below,answer] {\scriptsize \harm};}
	
	\draw (11.8,0) node[below,answer] {\scriptsize SIM swap success};  
	
	\foreach[count=\i] \harm in {Fake hw wallet received, Physical theats} {
		\draw (11.8+\i,0) node[below,answer] {\scriptsize \harm};
	}
	
	\path (0, 0)-- node[below=2.2cm] {Harm}(\xmax, 0);
	%y-axis
	\foreach \y in {0, 10, ..., 90} {
	\draw (\xmin,\y) -- +(-4pt, 0) node[left] {\scriptsize \y};}
	\path (\xmin, 0)-- node[left=25pt, rotate=90, anchor=center] {Respondents}(0, \ymax);

\end{tikzpicture}


==> fig/precaution.tex <==

%colors for the diverging likelihood scale (very unlikely - very likely)
%inspired by the gnuplot ColorBrewer PiYG scale
\definecolor{darkpurple}{HTML}{C51B7D}
\definecolor{mediumpurple}{HTML}{DE77AE}
\definecolor{mediumgreen}{HTML}{7FBC41}
\definecolor{darkgreen}{HTML}{4D9221}

%colors for the categorial scale (yes before, yes after, no)
% inspired by the Okabe-Ito scale
\definecolor{yesbefore}{rgb}{0.35,0.7,0.9}
\definecolor{yesafter}{rgb}{0,0.45,0.7}
\definecolor{no}{rgb}{0.80,0.40,0}

\begin{tikzpicture}[yscale=0.7,
					choice/.style={},
				 	label/.style={},
					line_prec/.style={},
								line_prec_a/.style={fill=yesbefore},
								line_prec_b/.style={fill=yesafter},
								line_prec_c/.style={fill=no},
					label_prec/.style={color=white},
								label_prec_a/.style={label_prec},
								label_prec_b/.style={label_prec},
								label_prec_c/.style={label_prec},
					line_int/.style={},
								line_int_a/.style={fill=darkpurple},
								line_int_b/.style={fill=mediumpurple},
								line_int_c/.style={},
								line_int_d/.style={fill=mediumgreen},
								line_int_e/.style={fill=darkgreen},
					label_int/.style={label},
								label_int_a/.style={label_int, white},
								label_int_b/.style={label_int, white},
								label_int_c/.style={label_int},
								label_int_d/.style={label_int, white},
								label_int_e/.style={label_int, white},
					callouts/.style={right,align=center,draw,fill=maincolor!20, drop shadow, rectangle callout},
						]
\footnotesize
\def\aax{0.2} %vspacebetween option label and bar A
\def\ax{4} %width of bar A (yes/no)
\def\ay{0.6} %height of bars
\def\abx{0.5} %vspace between bar A and B
\def\bx{7} %width of bar B (likelihood)
\begin{scope}[]
	\input{data/prec}
\end{scope}

%legend 
%%questions
\draw (barA)+(\ax/2,1.3) node[align=center] {Do you currently take the\\following precaution action?};
\draw (barB)+(\bx/2,\ay+1.3) node(question2)[align=center] {How likely is that you would take the following\\precaution action in response to this incident?};


%% Yes/No options
\draw (b)+(-2.2,0.33+\ay)  node {Using a...};
\draw (b)+(0,0.33+\ay) node[yesbefore!50!yesafter]{Yes};
\draw (no)+(0,0.33+\ay/2) node[no]{No};

%% likelihood scale
\draw (d)+(\abx,\ay+0.3) node[right, darkpurple,inner sep=0,outer sep=0]{Very unlikely};
\draw(i)+(0,0.3) node [left,darkgreen!50!black,inner sep=0,outer sep=0]{Very likely};

%% callouts
\visible<2>{\draw (yesb)++(-2.4,1) node [callouts, callout absolute pointer=(yesb)]{"Yes, I started doing it {\bf before} the breach."};}
\visible<3>{\draw (yesa)++(-2,1) node [callouts, callout absolute pointer=(yesa)]{"Yes, I started doing it {\bf after} the breach."};}
\visible<4>{\draw[black, thick, ->, shorten > = 1pt] (no)++(0.2,0) -- (question2.west);}
\end{tikzpicture}


==> fig/protection.tex <==

%min and max values
\def\xmax{18}
\def\ymax{65}
\def\xmin{0.25}	
\begin{tikzpicture}[xscale=0.75*14.6/\xmax, yscale=0.037*100/\ymax, answer/.style={anchor=north east, align=right,rotate=45, text width=3cm}]

	%n
	%\node at (\xmax-2,\ymax) {n=104}; %this has to be checked
	
	%data
	\begin{scope}[line width=12*14.6/\xmax, maincolor]
		\input{data/protec}
	\end{scope}

	%axis
	\draw[<->] (0\xmin, \ymax) -- (\xmin, 0) -- (\xmax, 0);
	
	%x-axis
	\foreach[count=\i] \x in {MFA, Changed email pwd, Authenticator apps, Changed crypto acc. pwd, Notified other affected, Password manager, Relocated seed, Transfer from hw wallet, Relocated hw wallet, Imp. home security, None, HW MFA, Transfer from exchange, Prevented SIM swap,  Data deletion request,I don't know, Increased awareness} {
		\draw (\i,0) node[below,answer] {\scriptsize \x};
	}
	
	\path (0, 0)-- node[below=2.2cm] {Protection}(\xmax, 0);
	%y-axis
	\foreach \y in {0, 10, ...,60} {
	\draw (\xmin,\y) -- +(-4pt, 0) node[left] {\scriptsize \y};}
	\path (\xmin, 0)-- node[left=25pt, rotate=90, anchor=center] {Respondents}(0, \ymax);
	
\end{tikzpicture}


==> fig/response.tex <==
%min and max values
\def\xmax{17}
\def\ymax{55}
\def\xmin{0.25}
\begin{tikzpicture}[xscale=0.75*14.6/\xmax, yscale=0.037*100/\ymax, answer/.style={anchor=north east, align=right,rotate=45, text width=3cm}]


	%n
	%\node at (\xmax-2,\ymax) {n=104}; %this has to be checked
	
	%data
	\begin{scope}[line width=12*14.6/\xmax, maincolor]
		\input{data/response}
	\end{scope}

	%axis
	\draw[<->] (\xmin, \ymax) -- (\xmin, 0) -- (\xmax, 0);
	
	%x-axis
	\foreach[count=\i] \x in {
		Company advice, 
		Followed disc. online,
		Time, Followed disc. website, Sought advice online, Sought advice community, No need, Shared exp. online, Sought advice peers, Sought advice company, Sought advice expert, I could not do anything, Spam management, Police, Other, I don't know} {
		\draw (\i,0) node[below,answer] {\scriptsize \x};
	}
	
	\path (0, 0)-- node[below=2.2cm] {Response}(\xmax, 0);
	%y-axis
	\foreach \y in {0, 10, ...,50} {
	\draw (\xmin,\y) -- +(-4pt, 0) node[left] {\scriptsize \y};}
	\path (\xmin, 0)-- node[left=25pt, rotate=90, anchor=center] {Respondents}(0, \ymax);
	
\end{tikzpicture}

